Reinforced Diffusion: Learning to Push the Limits of Anisotropic Diffusion for Image Denoising

Image denoising is an important problem in low-level vision and serves as a critical module for many image recovery tasks. Anisotropic diffusion is a wide family of image denoising approaches with promising performance. However, traditional anisotropic diffusion approaches use explicit diffusion operators which are not well adapted to complex image structures. As a result, their performance is limited compared to recent learning-based approaches. In this work, we describe a trainable anisotropic diffusion framework based on reinforcement learning. By modeling the denoising process as a series of naive diffusion actions with order learned by deep Q-learning, we propose an effective diffusion-based image denoiser. The diffusion actions selected by deep Q-learning at different iterations indeed composite a stochastic anisotropic diffusion process with strong adaptivity to different image structures, which enjoys improvement over the traditional ones. The proposed denoiser is applied to removing three types of often-seen noise. The experiments show that it outperforms existing diffusion-based methods and competes with the representative deep CNN-based methods.

==> SPLtex/mycom.tex <==
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{color}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{arydshln}
\usepackage{enumitem}

%%Path
\newcommand{\PathFig}{./fig}   %%Path of figures

%%Variable style
\newcommand{\matx}[1]{{\bm{#1}}} %%Matrix
\newcommand{\vect}[1]{{\bm{#1}}} %%Vector
\newcommand{\set}[1]{\mathbb{#1}} %%Set
\newcommand{\opt}[1]{\mathcal{#1}} %%Operator
%%Variable abbreviations (vectors)
\newcommand{\va}{\vect{a}}
\newcommand{\vb}{\vect{b}}
\newcommand{\vc}{\vect{c}}
\newcommand{\vd}{\vect{d}}
\newcommand{\ve}{\vect{e}}
\newcommand{\vf}{\vect{f}}
\newcommand{\vg}{\vect{g}}
\newcommand{\vh}{\vect{h}}
\newcommand{\vi}{\vect{i}}
\newcommand{\vj}{\vect{j}}
\newcommand{\vk}{\vect{k}}
\newcommand{\vl}{\vect{l}}
\newcommand{\vell}{\vect{\ell}}
\newcommand{\vm}{\vect{m}}
\newcommand{\vn}{\vect{n}}
\newcommand{\vo}{\vect{o}}
\newcommand{\vp}{\vect{p}}
\newcommand{\vq}{\vect{q}}
\newcommand{\vr}{\vect{r}}
\newcommand{\vs}{\vect{s}}
\newcommand{\vt}{\vect{t}}
\newcommand{\vu}{\vect{u}}
\newcommand{\vv}{\vect{v}}
\newcommand{\vw}{\vect{w}}
\newcommand{\vx}{\vect{x}}
\newcommand{\vy}{\vect{y}}
\newcommand{\vz}{\vect{z}}
\newcommand{\vZero}{\vect{0}}
\newcommand{\valpha}{\vect{\alpha}}
\newcommand{\vbeta}{\vect{\beta}}
\newcommand{\vgamma}{\vect{\gamma}}
\newcommand{\veta}{\vect{\eta}}
\newcommand{\vomega}{\vect{\omega}}
\newcommand{\vphi}{\vect{\phi}}
\newcommand{\vpsi}{\vect{\psi}}
%%Variable abbreviations (matrices)
\newcommand{\mA}{\matx{A}}
\newcommand{\mB}{\matx{B}}
\newcommand{\mC}{\matx{C}}
\newcommand{\mD}{\matx{D}}
\newcommand{\mE}{\matx{E}}
\newcommand{\mF}{\matx{F}}
\newcommand{\mG}{\matx{G}}
\newcommand{\mH}{\matx{H}}
\newcommand{\mI}{\matx{I}}
\newcommand{\mJ}{\matx{J}}
\newcommand{\mK}{\matx{K}}
\newcommand{\mL}{\matx{L}}
\newcommand{\mM}{\matx{M}}
\newcommand{\mN}{\matx{N}}
\newcommand{\mO}{\matx{O}}
\newcommand{\mP}{\matx{P}}
\newcommand{\mQ}{\matx{Q}}
\newcommand{\mR}{\matx{R}}
\newcommand{\mS}{\matx{S}}
\newcommand{\mT}{\matx{T}}
\newcommand{\mU}{\matx{U}}
\newcommand{\mV}{\matx{V}}
\newcommand{\mW}{\matx{W}}
\newcommand{\mX}{\matx{X}}
\newcommand{\mY}{\matx{Y}}
\newcommand{\mZ}{\matx{Z}}
\newcommand{\mPhi}{\matx{\Phi}}
\newcommand{\mPsi}{\matx{\Psi}}
\newcommand{\mZero}{\matx{0}}
%%Variable abbreviations (sets)
\newcommand{\sA}{\set{A}}
\newcommand{\sB}{\set{B}}
\newcommand{\sC}{\set{C}}
\newcommand{\sD}{\set{D}}
\newcommand{\sE}{\set{E}}
\newcommand{\sF}{\set{F}}
\newcommand{\sG}{\set{G}}
\newcommand{\sH}{\set{H}}
\newcommand{\sI}{\set{I}}
\newcommand{\sJ}{\set{J}}
\newcommand{\sK}{\set{K}}
\newcommand{\sL}{\set{L}}
\newcommand{\sM}{\set{M}}
\newcommand{\sN}{\set{N}}
\newcommand{\sO}{\set{O}}
\newcommand{\sP}{\set{P}}
\newcommand{\sQ}{\set{Q}}
\newcommand{\sR}{\set{R}}
\newcommand{\sS}{\set{S}}
\newcommand{\sT}{\set{T}}
\newcommand{\sU}{\set{U}}
\newcommand{\sV}{\set{V}}
\newcommand{\sW}{\set{W}}
\newcommand{\sX}{\set{X}}
\newcommand{\sY}{\set{Y}}
\newcommand{\sZ}{\set{Z}}
%%Variable abbreviations (operators)
\newcommand{\oA}{\opt{A}}
\newcommand{\oB}{\opt{B}}
\newcommand{\oC}{\opt{C}}
\newcommand{\oD}{\opt{D}}
\newcommand{\oE}{\opt{E}}
\newcommand{\oF}{\opt{F}}
\newcommand{\oG}{\opt{G}}
\newcommand{\oH}{\opt{H}}
\newcommand{\oI}{\opt{I}}
\newcommand{\oJ}{\opt{J}}
\newcommand{\oK}{\opt{K}}
\newcommand{\oL}{\opt{L}}
\newcommand{\oM}{\opt{M}}
\newcommand{\oN}{\opt{N}}
\newcommand{\oO}{\opt{O}}
\newcommand{\oP}{\opt{P}}
\newcommand{\oQ}{\opt{Q}}
\newcommand{\oR}{\opt{R}}
\newcommand{\oS}{\opt{S}}
\newcommand{\oT}{\opt{T}}
\newcommand{\oU}{\opt{U}}
\newcommand{\oV}{\opt{V}}
\newcommand{\oW}{\opt{W}}
\newcommand{\oX}{\opt{X}}
\newcommand{\oY}{\opt{Y}}
\newcommand{\oZ}{\opt{Z}}

\newcommand{\Range}{{\rm Range}}  %Range Space
\newcommand{\Null}{{\rm Null}}  %Null Space

\newcommand{\of}{f}    %NN
\newcommand{\stheta}{{\vect{\beta}}}  
\newcommand{\vtheta}{\vect{\theta}}
\newcommand{\vepsilon}{\vect{\epsilon}}
\newcommand{\sOmega}{\set{\Omega}}
\newcommand{\para}[1]{\vskip 1pt \noindent{\bfseries #1}\ }
\newcommand{\figpath}{fig}
\newcommand{\db}{{dB}}
%\newcommand{\bestun}[1]{{\textcolor[rgb]{0.00,0.00,1.00}{{#1}}}}		
%\newcommand{\bestsu}[1]{{\textcolor[rgb]{0.00,0.00,1.0}{{#1}}}}
\newcommand{\bestun}[1]{\underline{#1}}		
\newcommand{\bestsu}[1]{\underline{#1}}
\newcommand{\bestall}[1]{{\bf #1}}
\newcommand{\figtext}{\scriptsize}
\newcommand{\thl}[1]{\textbf{#1}}  %text highlight
%%Comments with highlights
\newcommand{\QYH}[1]{\textcolor[rgb]{1.00,0.00,0.00}{{#1}}} %For Quan Yuhui
\newcommand{\QXR}[1]{\textcolor[rgb]{0.00,0.00,1.00}{{#1}}} %For Pang Tongyao
%\newcommand{\QYH}[1]{{{#1}}} %For Quan Yuhui
\newcommand{\ST}[1]{\textcolor[rgb]{1.00,0.50,0.50}{{(ST:#1)}}} % For Students
\newcommand{\DIFF}[1]{\textcolor[rgb]{0.00,0.00,0.70}{{(#1)}}}
%%Word abbreviations
\newcommand{\ie}{{\it i.e.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\st}{\text{s.t.}\ \ }
\newcommand{\etal}{{\it et al.}}
\newcommand{\wrt}{{\it w.r.t.}\ }
%%

%argmin and argmax
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

%Proposition, etc.
\newtheorem{proposition}{Proposition}[]
\newtheorem{statement}{Statement}[]
\newtheorem{theorem}{Theorem}[]
\newtheorem{remark}{Remark}[]
\newtheorem{lemma}{Lemma}[]
\newtheorem{corollary}{Corollary}[]


